Node-Level Differentially Private Graph Neural Networks

Graph Neural Networks (GNNs) are a popular technique for modelling graph-structured data and computing node-level representations via aggregation of information from the neighborhood of each node. However, this aggregation implies an increased risk of revealing sensitive information, as a node can participate in the inference for multiple nodes. This implies that standard privacy-preserving machine learning techniques, such as differentially private stochastic gradient descent (DP-SGD) - which are designed for situations where each data point participates in the inference for one point only - either do not apply, or lead to inaccurate models. In this work, we formally define the problem of learning GNN parameters with node-level privacy, and provide an algorithmic solution with a strong differential privacy guarantee. We employ a careful sensitivity analysis and provide a non-trivial extension of the privacy-by-amplification technique to the GNN setting. An empirical evaluation on standard benchmark datasets demonstrates that our method is indeed able to learn accurate privacy-preserving GNNs which outperform both private and non-private methods that completely ignore graph information.

==> sampling-privacy.tex <==
\section{Privacy Analysis of $\mathsf{SAMPLE-SUBGRAPHS}$}
\label{app:sampling-privacy}
 
In this section, we analyze the step in $\mathsf{SAMPLE-SUBGRAPHS}$
in which nodes with high in-degree are `dropped'.

Consider any node $v \in G$. As each edge is sampled independently, the number of incoming edges to $v$ is given by the random variable $\widehat{d_v}$:
\begin{align*}
    \widehat{d_v} = \textup{Binomial}\left(d_v, \frac{K}{2 d_v}\right)
\end{align*}
where $d_v = |\mathbf{RE}_v|.$
Note that the expected number of incoming edges is only $\E[\widehat{d_v}] = \frac{K}{2}$.
The node $v$ is only dropped if the number of incoming edges exceeds $K$. This occurs with probability:
\begin{align*}
    \Pr\left[\widehat{d_v} > K\right]
    &= \Pr\left[\textup{Binomial}\left(d_v, \frac{K}{2 d_v}\right) > K\right] \\
    &= \sum_{r = K}^{d_v}\binom{d_v}{r} \left(\frac{K}{2 d_v}\right)^{r} \left(1 - \frac{K}{2 d_v}\right)^{d_v - r}.
\end{align*}
These probabilities are shown as a function of $d_v$ in \autoref{fig:drop-probabilities} for $K = 10$, which is
our recommended value of $K$ for $1$-layer GNNs.

\begin{figure}[htbp]
	\centering
    \includegraphics[width=.5\columnwidth]{figures/drop_probabilities.pdf}
    \caption{\textbf{Drop probabilities as a function of $d_v$ for $K = 10$.}}
    \label{fig:drop-probabilities}
\end{figure}

We see that nodes are dropped with very low probability.
For ogbn-arxiv, the distribution of $d_v$
shown in \autoref{fig:arxiv_indegree_distribution}
implies that only around $0.07\%$ of nodes are dropped.

\begin{figure}[htbp]
	\centering
    \includegraphics[width=.5\columnwidth]{figures/arxiv_degree_distribution.pdf}
    \caption{\textbf{In-degree over edges from training nodes ($d_v$) for ogbn-arxiv.}}
    \label{fig:arxiv_indegree_distribution}
\end{figure}

Consider a neighbouring graph $G'$ which consists of $G$ with an additional node $v'$.
In the worst case, $v'$ is connected to all of the nodes in $G$.
Despite this, the effect of adding $v'$ to the graph is small, in terms of the dropping probabilities.
This is because the addition of node $v'$ only increases $d_v$ by $1$, for the new edge
$(v, v')$ being added. However, $\E[\widehat{d_v}']$ continues to be $\frac{K}{2}$.
For node $v$, the dropping probability is now:
\begin{align*}
    \Pr\left[\widehat{d_v}' > K\right]
    &= \Pr\left[\textup{Binomial}\left(d_v + 1, \frac{K}{2 (d_v + 1)}\right) > K\right] \\
    &= \sum_{r = K}^{d_v + 1}\binom{d_v + 1}{r} \left(\frac{K}{2 (d_v + 1)}\right)^{r} \left(1 - \frac{K}{2 (d_v + 1)}\right)^{(d_v + 1) - r}.
\end{align*}

\begin{figure}[htbp]
	\centering
    \includegraphics[width=.5\columnwidth]{figures/drop_probabilities_delta.pdf}
    \caption{\textbf{Change in drop probabilities across node-level adjacent graphs
    as a function of $d_v$ for $K = 10$.}}
    \label{fig:drop_probabilities_delta}
\end{figure}

It is possible to compute the change in dropping probabilities numerically:
\begin{align*}
    \Delta(d_v, K) = \left|\Pr\left[\widehat{d_v}' > K\right] - \Pr\left[\widehat{d_v} > K\right]\right|
\end{align*}
as shown in \autoref{fig:drop_probabilities_delta}, again for $K = 10$.
We see that $\Delta(d_v, K)$ is bounded by $5\text{e-}4$
for this value of $K$.
In fact, for nodes $v$ such that $d_v + 1 \leq K$, we have $\Delta(d_v, K) = 0$.
For these nodes, there is no difference in the sampling outcome
even after adding a new node $v'$, as
they are not dropped in either $G$ or $G'$. 
Thus, there is no privacy loss for these nodes.

Thus, due to the minimal impact on privacy,
we have implemented the dropping of the nodes with
in-degree higher than $K$
in $\mathsf{SAMPLE-SUBGRAPHS}$ as a non differentially-private step.

